Experimental Demonstration of Frequency Regulation by Commercial Buildings - Part II: Results and Performance Evaluation

This paper is the second part of a two-part series presenting the results from an experimental demonstration of frequency regulation in a commercial building test facility. In Part I, we developed relevant building models and designed a hierarchical controller for reserve scheduling, building climate control and frequency regulation. In Part II, we introduce the communication architecture and experiment settings, and present extensive experimental results under frequency regulation. More specifically, we compute the day-ahead reserve capacity of the test facility under different assumptions and conditions. Furthermore, we demonstrate the ability of model predictive control to satisfy comfort constraints under frequency regulation, and show that fan speed control can track the fast-moving RegD signal of the Pennsylvania, Jersey, and Maryland Power Market (PJM) very accurately. In addition, we report the observed effects of frequency regulation on building control and provide suggestions for realworld implementation projects. Our results show that hierarchical control is appropriate for frequency regulation from commercial buildings.

==> commCtrlArch_v2.tex <==
\section{Control Approach} \label{sec_comm_arch}
FLEXLAB is controlled by a \ac{CWS} based on a predefined control sequence programmed in LabVIEW. From a TestStand National Instruments user interface, the operator can modify the setpoints of various control loops and observe the system's behavior in the chilled water loop, hot water loop, AHU, and conditioned rooms.
%This interface is very useful for infrequent update of control setpoints or monitoring purposes, but it cannot be used for frequency regulation because it would require constant human intervention.
%
% One possibility to automate the frequency regulation process would be to integrate our controllers within the existing LabVIEW environment. However, the option that was finally adopted was to use an existing scripting environment to send the control setpoints directly to the CWS.

External control commands can be sent to the CWS via a scripting environment, which allowed us to develop the frequency regulation controller externally in order to minimize conflicts with the LabVIEW code. Apart from the fan speed setpoint, all other control setpoints of the HVAC system were determined by the default controller in the CWS. Therefore, the designed controllers work complementarily to the existing ones and do not substitute them.
% \footnote{Overriding the default FLEXLAB controller increases the delay in the control loop (the average delay is $2.89$ seconds). The control delays are analyzed in Part II of this two-part paper.}
%
% The only modifications we did in the LabVIEW code were settings that did not change during the experiment (e.g., deactivation of the floor heating system).
% In addition, the SAT was fixed via the TestStand interface because there existed no relevant control point within the scripting environment.

The hierarchical controller consists of three levels: Level $1$: reserve scheduler, Level $2$: room climate controller, and Level $3$ frequency regulation controller. In this section, we provide a high-level introduction to the three control levels and explain the underlying communication architecture. The control sequences are shown in Fig.~\ref{fig:control_sequences}, whereas detailed mathematical formulations for the controllers will be provided in Section~\ref{CtrlDesign}.

\begin{figure}[t]
\centering
\includegraphics[width=0.5\textwidth]{control_sequences.pdf}
\vspace{-0.4cm}
\caption{Control sequences of the three levels of the hierarchical controller.} \label{fig:control_sequences}
\end{figure}

\subsubsection{Level $1$: Reserve Scheduler}
The goal of the reserve scheduler is to determine the reserve capacity that the building can reliably offer to the \ac{TSO}. In most markets, the reserve scheduling is performed one day ahead or one hour ahead of real-time operation. In this experiment, we assumed a day-ahead reserve scheduling occurring at $12.00$ of each day to determine the reserve capacity for the next day. The reserve scheduling is formulated as a multi-period robust optimization problem.
% In order to reliably provide the reserve capacity for any possible reserve request,
% \textbf{Mention somewhere that a similar scheduling (supervisory) control method was conceptually described in \cite{zhao2013evaluation} but without focusing on control design and analysis?}

\subsubsection{Level $2$: Room Climate Controller}
This zonal controller calculates the supply air flow rate setpoints that minimize energy consumption while ensuring occupant comfort under reserve provision. However, the control setpoints in the chilled water loop are determined by the default FLEXLAB controller. The room climate controller is implemented as a robust MPC that runs every $15$ minutes along with a Kalman filter.

\subsubsection{Level $3$: Frequency Regulation Controller}
The goal of this controller is to track the frequency regulation signal every $4$ seconds by modifying the fan power via fan speed control with a \ac{VFD}. For this purpose, we designed a switched controller comprised of a feedforward model-based controller and a feedback \ac{PI} controller.% with gain scheduling.

